Tetris is NP-hard even with $O(1)$ rows or columns

We prove that the classic falling-block video game Tetris (both survival and board clearing) remains NP-complete even when restricted to 8 columns, or to 4 rows, settling open problems posed over 15 years ago [BDH+04]. Our reduction is from 3-Partition, similar to the previous reduction for unrestricted board sizes, but with a better packing of buckets. On the positive side, we prove that 2-column Tetris (and 1-row Tetris) is polynomial. We also prove that the generalization of Tetris to larger $k$-omino pieces is NP-complete even when the board starts empty, even when restricted to 3 columns or 2 rows or constant-size pieces. Finally, we present an animated Tetris font.

==> tetris/figures/font/Makefile <==
all: \
  font_puzzle.pdf \
  font_solved.pdf \
  font_anim_1.pdf \
  font_anim_2.pdf \
  font_anim_3.pdf \
  font_anim_4.pdf \
  font_anim_5.pdf \
  font_anim_6.pdf \
  font_anim_7.pdf

%.pdf: %.svg
	inkscape -A $@ $<

